The Diffeomorphism Field

Integration of Kirillov form on a coadjoint orbit of Virasoro algebra yields the coupling of a background field to Polyakov's two dimensional quantum gravity. This background field is used to be called the diffeomorphism field. Einstein's gravity is dynamically trivial in two dimensions. Moreover, the diffeomorphism field can be interpreted as the gravitational analog of a Yang-Mills field. This raises the question of whether the diffeomorphism field exists in higher dimensions, and plays an essential role in gravity. With this motivation, several dynamical theories for the diffeomorphism field have been constructed by mimicking construction of Yang-Mills theory from Kac-Moody algebra. This thesis constitutes a further development for obtaining a consistent dynamical theory of the diffeomorphism field. The previously proposed theories are thoroughly examined, certain subtleties and problems in them have been discovered and made apparent. Some of these problems have been solved, and for others possible routes to follow have been laid down. Finally, alternative geometric approaches are investigated.

==> Symbols.tex <==


\section*{\begin{center}
	\normalsize{LIST OF ABBREVIATIONS}
	\end{center}}




\all{
& \text{KM}  &&\text{Kac-Moody} \\
& \text{YM}  &&\text{Yang-Mills} \\ 
& \text{WZW} && \text{Wess-Zumino-Witten} \\ 
& \text{P2DG} &&\text{Polyakov-2D-Gravity}
\\ 
& \text{diff field}  &&\text{diffeomorphism field}  \\
& \text{$N$D} &&\text{$N$-dimensional}
\\
& \text{PB} &&\text{Poisson bracket}
\\
& \text{GCT} && \text{general coordinate transformation}
\\
& \text{LCC} && \text{lightcone coordinates}
\\
& \text{LCG} && \text{lightcone gauge}
\\
& \text{EL} && \text{Euler-Lagrange}
\\
& \text{EP} && \text{Euler-Poincare}
}









==> dedication.tex <==
To My Mother
%(Prior to your first thesis deposit, delete this text and type your dedication here.  The entire dedication should be single spaced and centered vertically and horizontally on the page.  This text may be altered between first and final deposit.)\\
%
%THIS PAGE IS OPTIONAL


==> publicAbstract.tex <==
    
In 1687, Isaac Newton proposed a theory of gravity that successfully explained  phenomena ranging from the free-fall of an object to the orbiting of the planets around the Sun. 
However, improved astronomical observations  showed both qualitative and quantitative problems with Newton's theory. The bending of light and the observed perihelion shift of Mercury are among the phenomena for which Newton's theory could not provide an accurate explanation. 

In 1915, Albert Einstein proposed another theory of gravity, called general relativity, which is entirely different in its interpretation of gravity, yet reduces to Newton's theory for weak gravitational interaction.   General relativity has provided a successful description of gravity in  the Solar system and explained the large scale structure of the Universe.

However, new problems arose for which general relativity could not provide a satisfactory explanation, in particular, the dark energy/matter problem. Visible matter is insufficient to explain the observed expansion rate of the Universe.  Moreover, Einstein's theory is not compatible with quantum mechanics, by now, the most successful theory of physics. Hence, a further extension is needed. 

A method frequently used in theoretical physics is to study models in lower dimensions where normally inaccessible mathematical features are present. Conformal field theories in two dimensions, and a particular subset of them blended with supersymmetry,  string theories have been the central theme in theoretical physics in the last thirty years. This thesis is on the diffeomorphism field,  which  is discovered in the study of two-dimensional quantum gravity, and is being developed in hope of solving some of the problems stated  above.


==> symbols.tex <==


\section*{\begin{center}
	\normalsize{LIST OF ABBREVIATIONS}
	\end{center}}




\all{
& \text{KM}  &&\text{Kac-Moody} \\
& \text{YM}  &&\text{Yang-Mills} \\ 
& \text{WZW} && \text{Wess-Zumino-Witten} \\ 
& \text{P2DG} &&\text{Polyakov-2D-Gravity}
\\ 
& \text{diff field}  &&\text{diffeomorphism field}  \\
& \text{$N$D} &&\text{$N$-dimensional}
\\
& \text{PB} &&\text{Poisson bracket}
\\
& \text{GCT} && \text{general coordinate transformation}
\\
& \text{LCC} && \text{lightcone coordinates}
\\
& \text{LCG} && \text{lightcone gauge}
\\
& \text{EL} && \text{Euler-Lagrange}
\\
& \text{EP} && \text{Euler-Poincare}
}









==> thesisAbstract.tex <==

Integration of Kirillov form on a coadjoint orbit of Virasoro algebra yields the coupling of a background field to Polyakov's two dimensional quantum gravity. This background field is used to be called the diffeomorphism field. Einstein's gravity is dynamically trivial in two dimensions. Moreover,  the diffeomorphism field can be interpreted as the gravitational analog of a Yang-Mills field. This raises the question of whether the diffeomorphism field exists in higher dimensions, and plays an essential role in gravity. With this motivation, several dynamical theories for the diffeomorphism field have been constructed by mimicking construction of Yang-Mills theory from Kac-Moody algebra. 

This thesis constitutes a further development for obtaining a consistent dynamical theory of the diffeomorphism field. The previously proposed theories are thoroughly examined, certain subtleties and problems in them have been discovered and made apparent. Some of these problems have been solved, and for others possible routes to follow have been laid down. Finally, alternative geometric approaches  are investigated.

==> thesisAck.tex <==
First of all, I would like to  thank my advisor Vincent Rodgers for accepting me into D$\&$G group and introducing me to the diffeomorphism field project. He has always been understanding and supportive when I had fallbacks. I also would like to thank Haluk Beker, my MS advisor, for introducing me to doing research.

I would like to thank my committee members Wayne Polyzou, Hao Fang, and Mary Hall Reno; especially Yannick Meurice for his challenging questions and valuable suggestions, and Yasar Onel for his continuous support and guidance throughout my graduate years.

I would like to thank  new and old D$\&$G group  members Kenneth Heitritter, Sam Brensinger, Nicholas Jones, Catherine Whiting; especially Bradly Button, Chris Doran and Tuna Yildirim for their friendship and contribution to my intellect. 

I would like to thank Emrah Tiras and Suleyman Durgut for their friendship; Marc Herrmann for his friendship and for our illuminating discussions thanks to his critical thinking skills.

Among all  my friends here, Burak Bilki, Wyatt VanGlasnap, and Calvin Mera have a distinct place. They have always been there when I needed and a source of joy in my graduate years; and Cuneyt Sahin with whom we have been friends for fifteen years, and who was the main reason I chose the  University of Iowa for PhD. He had a huge impact on my intellectual development.

Finally, I would like to thank my family. Although we have been ten thousand kilometers apart, I have always felt their support. Thanks to the  summer visits to Turkey I  started every year fresh. Their presence has been the main drive I had to complete PhD. 

